MP3: Movement Primitive-Based (Re-)Planning Policy

We introduce a novel deep reinforcement learning (RL) approach called Movement Primitive-based Planning Policy (MP3). By integrating movement primitives (MPs) into the deep RL framework, MP3 enables the generation of smooth trajectories throughout the whole learning process while effectively learning from sparse and non-Markovian rewards. Additionally, MP3 maintains the capability to adapt to changes in the environment during execution. Although many early successes in robot RL have been achieved by combining RL with MPs, these approaches are often limited to learning single stroke-based motions, lacking the ability to adapt to task variations or adjust motions during execution. Building upon our previous work, which introduced an episode-based RL method for the non-linear adaptation of MP parameters to different task variations, this paper extends the approach to incorporating replanning strategies. This allows adaptation of the MP parameters throughout motion execution, addressing the lack of online motion adaptation in stochastic domains requiring feedback. We compared our approach against state-of-the-art deep RL and RL with MPs methods. The results demonstrated improved performance in sophisticated, sparse reward settings and in domains requiring replanning.

==> contents/mp_related_work.tex <==
\acrfullpl{mp} are a widely used tool for motion representation and generation in robotics. 
They are used as building blocks for movements, allowing for the modulate of motion behavior and the creation of more complex movements through combination or concatenation. 
With their concise parameterization and flexibility, \acrshortpl{mp} have become a popular choice in imitation and reinforcement learning.
In this work, we focus on using trajectory-based movement representations, as discussed in works by \cite{Schaal2006, Ijspeert2013, Paraschos2013, li2022prodmps} for \acrshort{rl}.
Given a parameter vector, these representations generate desired trajectories for the agent to follow, and the goal is often to optimize the parameter vector or its distribution to improve the resulting movements.

One popular way to form up a desired trajectory is via \acrshortpl{promp}. As described in \cite{Paraschos2013}, the trajectory $\bm{\lambda}$ is represented by a linear basis function model and its behaviour is modulated by a weight vector, as
\begin{equation}
    y(t) = \bm{\Phi}^\intercal(t) \bm{w},  \quad \bm{\lambda} = [y_t]_{t=0:T} = \bm{\Phi}_{0:T}^\intercal \bm{w} 
\end{equation}
where $y(t)$ is the trajectory position at time step $t$, $\bm{w}$ a time-independent weight vector and $\bm{\Phi}$ some pre-defined time-dependent basis functions, e.g., RBF basis. 
Due to the simplicity of the linear basis function representation, \acrshortpl{promp} allows fast trajectory computation and enables modeling the trajectory's statistics from the weight vector's distribution. Such statistics often include temporal correlations of the trajectories and the motion correlations across different \acrshort{dof}.
One of the key limitations of \acrshortpl{promp} as a representation method is its lack of smoothness in trajectory replanning and concatenation. This is because the motion dynamics are not taken into consideration in the linear basis function representation, making it impossible to ensure a desired starting state by merely adjusting the weights vector $\bm{w}$. 
This lack of smoothness and inability to adjust the trajectory's start state poses limitations in the practical application of \acrshortpl{promp}, especially in situations where responsiveness to changes in the environment, or the need for improving sample efficiency are important considerations.

The necessity of modeling dynamics in movement representation are often addressed by another group of \acrshortpl{mp}, \ie, \acrshortpl{dmp} \citep{Schaal2006, Ijspeert2013}. \acrshortpl{dmp} form a trajectory by integrating a dynamic system, providing smooth replanning of both position and velocity (\cite{brandherm2019learning, ginesi2019knowledge, lee2020trajectory}). However, this smoothness comes at a computational cost, as \acrshortpl{dmp} require online numerical integration to compute a trajectory. Moreover, when integrating \acrshortpl{dmp} with deep \acrshortpl{nn}, the forward and backward pass of the neural networks become coupled with the numerical integration (\cite{Bahl2020, gams2018deep, ridge2020training}), which makes the usage of such deep \acrshortpl{dmp} model complex and slow. 

To combine the advantages and address the limitations of both \acrshortpl{mp} methodologies, \cite{li2022prodmps} recently proposed \acrfullpl{pdmp} by sovling the \acrshortpl{dmp}' underlying \acrfull{ode}, and transformed the expensive online numerical integration into position and velocity basis functions, which can be shared by all trajectories and computed offline.
The resulting representation of trajectory position and velocity in \acrshortpl{pdmp} takes a similar form of \acrshortpl{promp}, as:
\begin{equation}
    y(t) = c_1y_1(t) + c_2y_2(t) + \ipb(t)^\intercal \bm{w}_g, \quad \dot{y}(t)=c_1\dot{y}_1(t) + c_2\dot{y}_2(t) + \ivb(t)^\intercal\bm{w}_g, \label{eq:prodmp}
\end{equation}
where the $y_1$ and $y_2$ are the two linearly independent complementary functions of \acrshortpl{dmp}'s governing ODE, with $\dot{y}_1$, $\dot{y}_2$ their corresponding derivatives w.r.t. time. The coefficients $c_1$ and $c_2$ shared by both position and velocity representations are determined by solving an initial condition problem of the \acrshort{ode}. $\ipb$ and $\ivb$ are the position and velocity basis functions resepectively which can be computed only once offline and later used as constant functions. The vector $\bm{w}_g$ in both equations concatenates the \acrshortpl{dmp}'s original weights $\bm{w}$ and goal $g$ into one vector. 
We offered a brief derivation of these equations in Appendix \ref{app:pdmp}, while we refer to the original paper (\cite{li2022prodmps}) for the exact details.

In our current work, we use the \acrshortpl{pdmp} model as our trajectory generator due to its ability to ensure smooth replanning with low computational cost.

% \todo{Bruce: I do not see any other reasons to use ProDMP in the current work.}









% Bruce commented all the old stuff in below


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % ProMP
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% One popular way to represent a desired trajectory is via \acrshortpl{promp} \citep{Paraschos2013}.
% They establish a framework to model \acrshortpl{mp} as trajectory distributions which can capture correlation over time and between the trajectory dimensions. 
% For this work we, however, only consider the mean of that trajectory distribution and refer the reader to \citet{Paraschos2013} for further details. 
% \acrshortpl{promp} are able to directly model a 1-degree-of-freedom trajectory as $\bm{\lambda} = [y_t]_{t=0:T} = \bm{\Phi}_{0:T}^\intercal \bm{w}$, where $\bm{w}$ is a learned weight vector.
% % The probability of observing a 1-degree-of-freedom trajectory $\bm{\lambda} = [y_t]_{t=0:T}$, given an underlying weight vector distribution $p(\bm{w}) \sim \mathcal{N}(\bm{w}|\bm{\mu_w}, \bm{\Sigma_w})$, can be expressed as a linear basis function model,
% % \begin{equation}
% %     \bm{\lambda} = \bm{\Phi}_{0:T}^\intercal \bm{w} + \epsilon_{y}, \quad\quad 
% %     p(\bm{\lambda} ; \bm{\mu_w}, \bm{\Sigma_w}) = \mathcal{N}(\bm{\lambda} ~|~ \bm{\Phi}_{0:T}^\intercal\bm{\mu_w}, ~\bm{\Phi}_{0:T}^\intercal \bm{\Sigma_w} \bm{\Phi}_{0:T}~+ \sigma_y^2 \bm{I}),   
% %     \label{eq:promp_p_of_y}
% % \end{equation}
% % where $\epsilon_{y}$ is zero mean white noise with variance $\sigma_y^2$. 
% Each column in the matrix $\bm{\Phi}_{0:T}$ contains the basis functions of a single time step $t$. 
% % Exploration is already taking placWe on the policy level by sampling weights $\bm{w}$.

% One core issue \acrshortpl{promp} have is, they are not able to guarantee smoothness when replanning, \ie adjusting the weights $\bm{w}$, and thus the trajectory, during execution. 
% This makes replanning with \acrshortpl{promp} less desireable although it is necessary to \eg react to changes in the environment, moving objects, failure, or just to improve the sample efficiency.
% While \acrshortpl{dmp} are able to guarantee smoothness when replanning, they are computationally expensive due to their online numerical integration. 
% Hence, the recently introduced \acrfullpl{pdmp} \cite{li2022prodmps} are well suited for our use case. 
% They combine the smoothness guarantee of \acrshortpl{dmp} with the computationally efficiency of \acrshortpl{promp}. 


==> jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``MP3: Movement Primitives-Based (Re-)Planning Policy'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies how to effectively integrate Movement Primitives(MP) into the deep reinforcement learning framework. This is important in robot learning as it enables exploration at the trajectory level, leading to smooth trajectory generation throughout the whole learning process. Furthermore, this method facilitates effective learning from sparse and non-Markovian rewards.

This paper extends our work of ``Deep Black-Box Reinforcement Learning with Movement Primitives'' (CoRL 2022: 1244-1265) by addressing the lack of online motion adaptation in stochastic domains requiring feedback.

We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item George Konidaris, Brown University, USA (gdk@cs.brown.edu)
    \item Martha White, University of Alberta, Canada (whitem@ualberta.ca)
    \item Marc Bellemare, Google Research, Canada (bellemare@google.com)
    \item Csaba Szepesvari, University of Alberta, Canada (csaba.szepesvari@gmail.com)
 %   \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item Carlo DEramo, University of Würzburg, Germany (carlo.deramo@uni-wuerzburg.de)
    \item Marcello Restelli, Politecnico di Milano, Italy (marcello.restelli@polimi.it)
    \item David Abel, DeepMind, London (dmabel@deepmind.com)
    \item Dylan Foster, Microsoft Research Lab, USA (dylanfoster@microsoft.com)
    \item Rahul Kiadambi, Amazon Search and AI, USA (rkidambi@uw.edu)
\end{itemize}

Our submission has the following keywords: Movement primitives, deep reinforcement learning, trust region, robot learning, sparse and non-Markovian rewards.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

Fabian Otto* (Bosch Center for Artificial Intelligence, Germany)\\
Hongyi Zhou* (Karlsruhe Institute of Technology, Germany)\\
Onur Celik  (Karlsruhe Institute of Technology, Germany)\\
Ge Li (Karlsruhe Institute of Technology, Germany)\\
Rudolf Lioutikov (Karlsruhe Institute of Technology, Germany)\\
Gerhard Neumann (Karlsruhe Institute of Technology, Germany)

\end{document}








































==> tables/ablation_dense_tikz.tex <==
\begin{tikzpicture}
  \begin{axis}[enlargelimits=false,colorbar,colormap/Purples, title=Dense Reward,
     xlabel = {Replanning Steps}, ylabel = {Number of Basis},
     ytick={0, 1, 2, 3, 4, 5, 6},
     xtick={0, 1, 2, 3, 4, 5, 6},
     xticklabels={{1}, {2}, {5}, {10}, {25}, {50}, {100}}]
    \addplot [matrix plot,
    point meta=explicit, point meta min=0.0, point meta max=1.0]
      coordinates {
(0, 0) [0.55] (1, 0) [0.75] (2, 0) [0.68] (3, 0) [0.55] (4, 0) [0.47] (5, 0) [0.15] (6, 0) [0.00] 

(0, 1) [0.75] (1, 1) [0.82] (2, 1) [0.82] (3, 1) [0.68] (4, 1) [0.68] (5, 1) [0.38] (6, 1) [0.05] 

(0, 2) [0.75] (1, 2) [0.82] (2, 2) [0.85] (3, 2) [0.88] (4, 2) [0.70] (5, 2) [0.55] (6, 2) [0.17] 

(0, 3) [0.70] (1, 3) [0.85] (2, 3) [0.85] (3, 3) [0.80] (4, 3) [0.75] (5, 3) [0.85] (6, 3) [0.47] 

(0, 4) [0.78] (1, 4) [0.82] (2, 4) [0.82] (3, 4) [0.88] (4, 4) [0.80] (5, 4) [0.82] (6, 4) [0.65] 

(0, 5) [0.70] (1, 5) [0.75] (2, 5) [0.82] (3, 5) [0.90] (4, 5) [0.75] (5, 5) [0.78] (6, 5) [0.68] 

(0, 6) [0.70] (1, 6) [0.70] (2, 6) [0.75] (3, 6) [0.85] (4, 6) [0.82] (5, 6) [0.78] (6, 6) [0.62] 
      };
  \end{axis}
\end{tikzpicture}

==> tables/ablation_sparse2_tikz.tex <==
\begin{tikzpicture}
  \begin{axis}[enlargelimits=false,colorbar,colormap/Purples, title=Sparse Reward,
     xlabel = {Replanning Steps}, ylabel = {Number of Basis},
     ytick={0, 1, 2, 3, 4, 5, 6},
     xtick={0, 1, 2, 3, 4, 5, 6},
     xticklabels={{1}, {2}, {5}, {10}, {25}, {50}, {100}}]
    \addplot [matrix plot,
    point meta=explicit, point meta min=0.0, point meta max=1.0]
      coordinates {
(0, 0) [0.00] (1, 0) [0.00] (2, 0) [0.00] (3, 0) [0.00] (4, 0) [0.00] (5, 0) [0.00] (6, 0) [0.00] 

(0, 1) [0.00] (1, 1) [0.00] (2, 1) [0.82] (3, 1) [0.38] (4, 1) [0.68] (5, 1) [0.45] (6, 1) [0.00] 

(0, 2) [0.72] (1, 2) [0.90] (2, 2) [0.90] (3, 2) [0.90] (4, 2) [0.78] (5, 2) [0.30] (6, 2) [0.12] 

(0, 3) [0.70] (1, 3) [0.93] (2, 3) [0.93] (3, 3) [0.95] (4, 3) [0.88] (5, 3) [0.65] (6, 3) [0.43] 

(0, 4) [0.75] (1, 4) [0.93] (2, 4) [0.85] (3, 4) [0.95] (4, 4) [0.95] (5, 4) [0.78] (6, 4) [0.70] 

(0, 5) [0.70] (1, 5) [0.85] (2, 5) [0.70] (3, 5) [0.82] (4, 5) [0.95] (5, 5) [0.80] (6, 5) [0.65] 

(0, 6) [0.57] (1, 6) [0.68] (2, 6) [0.53] (3, 6) [0.72] (4, 6) [0.90] (5, 6) [0.93] (6, 6) [0.57] 

      };
  \end{axis}
\end{tikzpicture}

==> tables/ablation_success_rate_sparse2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkslategray38}{RGB}{38,38,38}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap={mymap}{[1pt]
 rgb(0pt)=(0.01060815,0.01808215,0.10018654);
  rgb(1pt)=(0.01428972,0.02048237,0.10374486);
  rgb(2pt)=(0.01831941,0.0229766,0.10738511);
  rgb(3pt)=(0.02275049,0.02554464,0.11108639);
  rgb(4pt)=(0.02759119,0.02818316,0.11483751);
  rgb(5pt)=(0.03285175,0.03088792,0.11863035);
  rgb(6pt)=(0.03853466,0.03365771,0.12245873);
  rgb(7pt)=(0.04447016,0.03648425,0.12631831);
  rgb(8pt)=(0.05032105,0.03936808,0.13020508);
  rgb(9pt)=(0.05611171,0.04224835,0.13411624);
  rgb(10pt)=(0.0618531,0.04504866,0.13804929);
  rgb(11pt)=(0.06755457,0.04778179,0.14200206);
  rgb(12pt)=(0.0732236,0.05045047,0.14597263);
  rgb(13pt)=(0.0788708,0.05305461,0.14995981);
  rgb(14pt)=(0.08450105,0.05559631,0.15396203);
  rgb(15pt)=(0.09011319,0.05808059,0.15797687);
  rgb(16pt)=(0.09572396,0.06050127,0.16200507);
  rgb(17pt)=(0.10132312,0.06286782,0.16604287);
  rgb(18pt)=(0.10692823,0.06517224,0.17009175);
  rgb(19pt)=(0.1125315,0.06742194,0.17414848);
  rgb(20pt)=(0.11813947,0.06961499,0.17821272);
  rgb(21pt)=(0.12375803,0.07174938,0.18228425);
  rgb(22pt)=(0.12938228,0.07383015,0.18636053);
  rgb(23pt)=(0.13501631,0.07585609,0.19044109);
  rgb(24pt)=(0.14066867,0.0778224,0.19452676);
  rgb(25pt)=(0.14633406,0.07973393,0.1986151);
  rgb(26pt)=(0.15201338,0.08159108,0.20270523);
  rgb(27pt)=(0.15770877,0.08339312,0.20679668);
  rgb(28pt)=(0.16342174,0.0851396,0.21088893);
  rgb(29pt)=(0.16915387,0.08682996,0.21498104);
  rgb(30pt)=(0.17489524,0.08848235,0.2190294);
  rgb(31pt)=(0.18065495,0.09009031,0.22303512);
  rgb(32pt)=(0.18643324,0.09165431,0.22699705);
  rgb(33pt)=(0.19223028,0.09317479,0.23091409);
  rgb(34pt)=(0.19804623,0.09465217,0.23478512);
  rgb(35pt)=(0.20388117,0.09608689,0.23860907);
  rgb(36pt)=(0.20973515,0.09747934,0.24238489);
  rgb(37pt)=(0.21560818,0.09882993,0.24611154);
  rgb(38pt)=(0.22150014,0.10013944,0.2497868);
  rgb(39pt)=(0.22741085,0.10140876,0.25340813);
  rgb(40pt)=(0.23334047,0.10263737,0.25697736);
  rgb(41pt)=(0.23928891,0.10382562,0.2604936);
  rgb(42pt)=(0.24525608,0.10497384,0.26395596);
  rgb(43pt)=(0.25124182,0.10608236,0.26736359);
  rgb(44pt)=(0.25724602,0.10715148,0.27071569);
  rgb(45pt)=(0.26326851,0.1081815,0.27401148);
  rgb(46pt)=(0.26930915,0.1091727,0.2772502);
  rgb(47pt)=(0.27536766,0.11012568,0.28043021);
  rgb(48pt)=(0.28144375,0.11104133,0.2835489);
  rgb(49pt)=(0.2875374,0.11191896,0.28660853);
  rgb(50pt)=(0.29364846,0.11275876,0.2896085);
  rgb(51pt)=(0.29977678,0.11356089,0.29254823);
  rgb(52pt)=(0.30592213,0.11432553,0.29542718);
  rgb(53pt)=(0.31208435,0.11505284,0.29824485);
  rgb(54pt)=(0.31826327,0.1157429,0.30100076);
  rgb(55pt)=(0.32445869,0.11639585,0.30369448);
  rgb(56pt)=(0.33067031,0.11701189,0.30632563);
  rgb(57pt)=(0.33689808,0.11759095,0.3088938);
  rgb(58pt)=(0.34314168,0.11813362,0.31139721);
  rgb(59pt)=(0.34940101,0.11863987,0.3138355);
  rgb(60pt)=(0.355676,0.11910909,0.31620996);
  rgb(61pt)=(0.36196644,0.1195413,0.31852037);
  rgb(62pt)=(0.36827206,0.11993653,0.32076656);
  rgb(63pt)=(0.37459292,0.12029443,0.32294825);
  rgb(64pt)=(0.38092887,0.12061482,0.32506528);
  rgb(65pt)=(0.38727975,0.12089756,0.3271175);
  rgb(66pt)=(0.39364518,0.12114272,0.32910494);
  rgb(67pt)=(0.40002537,0.12134964,0.33102734);
  rgb(68pt)=(0.40642019,0.12151801,0.33288464);
  rgb(69pt)=(0.41282936,0.12164769,0.33467689);
  rgb(70pt)=(0.41925278,0.12173833,0.33640407);
  rgb(71pt)=(0.42569057,0.12178916,0.33806605);
  rgb(72pt)=(0.43214263,0.12179973,0.33966284);
  rgb(73pt)=(0.43860848,0.12177004,0.34119475);
  rgb(74pt)=(0.44508855,0.12169883,0.34266151);
  rgb(75pt)=(0.45158266,0.12158557,0.34406324);
  rgb(76pt)=(0.45809049,0.12142996,0.34540024);
  rgb(77pt)=(0.46461238,0.12123063,0.34667231);
  rgb(78pt)=(0.47114798,0.12098721,0.34787978);
  rgb(79pt)=(0.47769736,0.12069864,0.34902273);
  rgb(80pt)=(0.48426077,0.12036349,0.35010104);
  rgb(81pt)=(0.49083761,0.11998161,0.35111537);
  rgb(82pt)=(0.49742847,0.11955087,0.35206533);
  rgb(83pt)=(0.50403286,0.11907081,0.35295152);
  rgb(84pt)=(0.51065109,0.11853959,0.35377385);
  rgb(85pt)=(0.51728314,0.1179558,0.35453252);
  rgb(86pt)=(0.52392883,0.11731817,0.35522789);
  rgb(87pt)=(0.53058853,0.11662445,0.35585982);
  rgb(88pt)=(0.53726173,0.11587369,0.35642903);
  rgb(89pt)=(0.54394898,0.11506307,0.35693521);
  rgb(90pt)=(0.5506426,0.11420757,0.35737863);
  rgb(91pt)=(0.55734473,0.11330456,0.35775059);
  rgb(92pt)=(0.56405586,0.11235265,0.35804813);
  rgb(93pt)=(0.57077365,0.11135597,0.35827146);
  rgb(94pt)=(0.5774991,0.11031233,0.35841679);
  rgb(95pt)=(0.58422945,0.10922707,0.35848469);
  rgb(96pt)=(0.59096382,0.10810205,0.35847347);
  rgb(97pt)=(0.59770215,0.10693774,0.35838029);
  rgb(98pt)=(0.60444226,0.10573912,0.35820487);
  rgb(99pt)=(0.61118304,0.10450943,0.35794557);
  rgb(100pt)=(0.61792306,0.10325288,0.35760108);
  rgb(101pt)=(0.62466162,0.10197244,0.35716891);
  rgb(102pt)=(0.63139686,0.10067417,0.35664819);
  rgb(103pt)=(0.63812122,0.09938212,0.35603757);
  rgb(104pt)=(0.64483795,0.0980891,0.35533555);
  rgb(105pt)=(0.65154562,0.09680192,0.35454107);
  rgb(106pt)=(0.65824241,0.09552918,0.3536529);
  rgb(107pt)=(0.66492652,0.09428017,0.3526697);
  rgb(108pt)=(0.67159578,0.09306598,0.35159077);
  rgb(109pt)=(0.67824099,0.09192342,0.3504148);
  rgb(110pt)=(0.684863,0.09085633,0.34914061);
  rgb(111pt)=(0.69146268,0.0898675,0.34776864);
  rgb(112pt)=(0.69803757,0.08897226,0.3462986);
  rgb(113pt)=(0.70457834,0.0882129,0.34473046);
  rgb(114pt)=(0.71108138,0.08761223,0.3430635);
  rgb(115pt)=(0.7175507,0.08716212,0.34129974);
  rgb(116pt)=(0.72398193,0.08688725,0.33943958);
  rgb(117pt)=(0.73035829,0.0868623,0.33748452);
  rgb(118pt)=(0.73669146,0.08704683,0.33543669);
  rgb(119pt)=(0.74297501,0.08747196,0.33329799);
  rgb(120pt)=(0.74919318,0.08820542,0.33107204);
  rgb(121pt)=(0.75535825,0.08919792,0.32876184);
  rgb(122pt)=(0.76145589,0.09050716,0.32637117);
  rgb(123pt)=(0.76748424,0.09213602,0.32390525);
  rgb(124pt)=(0.77344838,0.09405684,0.32136808);
  rgb(125pt)=(0.77932641,0.09634794,0.31876642);
  rgb(126pt)=(0.78513609,0.09892473,0.31610488);
  rgb(127pt)=(0.79085854,0.10184672,0.313391);
  rgb(128pt)=(0.7965014,0.10506637,0.31063031);
  rgb(129pt)=(0.80205987,0.10858333,0.30783);
  rgb(130pt)=(0.80752799,0.11239964,0.30499738);
  rgb(131pt)=(0.81291606,0.11645784,0.30213802);
  rgb(132pt)=(0.81820481,0.12080606,0.29926105);
  rgb(133pt)=(0.82341472,0.12535343,0.2963705);
  rgb(134pt)=(0.82852822,0.13014118,0.29347474);
  rgb(135pt)=(0.83355779,0.13511035,0.29057852);
  rgb(136pt)=(0.83850183,0.14025098,0.2876878);
  rgb(137pt)=(0.84335441,0.14556683,0.28480819);
  rgb(138pt)=(0.84813096,0.15099892,0.281943);
  rgb(139pt)=(0.85281737,0.15657772,0.27909826);
  rgb(140pt)=(0.85742602,0.1622583,0.27627462);
  rgb(141pt)=(0.86196552,0.16801239,0.27346473);
  rgb(142pt)=(0.86641628,0.17387796,0.27070818);
  rgb(143pt)=(0.87079129,0.17982114,0.26797378);
  rgb(144pt)=(0.87507281,0.18587368,0.26529697);
  rgb(145pt)=(0.87925878,0.19203259,0.26268136);
  rgb(146pt)=(0.8833417,0.19830556,0.26014181);
  rgb(147pt)=(0.88731387,0.20469941,0.25769539);
  rgb(148pt)=(0.89116859,0.21121788,0.2553592);
  rgb(149pt)=(0.89490337,0.21785614,0.25314362);
  rgb(150pt)=(0.8985026,0.22463251,0.25108745);
  rgb(151pt)=(0.90197527,0.23152063,0.24918223);
  rgb(152pt)=(0.90530097,0.23854541,0.24748098);
  rgb(153pt)=(0.90848638,0.24568473,0.24598324);
  rgb(154pt)=(0.911533,0.25292623,0.24470258);
  rgb(155pt)=(0.9144225,0.26028902,0.24369359);
  rgb(156pt)=(0.91717106,0.26773821,0.24294137);
  rgb(157pt)=(0.91978131,0.27526191,0.24245973);
  rgb(158pt)=(0.92223947,0.28287251,0.24229568);
  rgb(159pt)=(0.92456587,0.29053388,0.24242622);
  rgb(160pt)=(0.92676657,0.29823282,0.24285536);
  rgb(161pt)=(0.92882964,0.30598085,0.24362274);
  rgb(162pt)=(0.93078135,0.31373977,0.24468803);
  rgb(163pt)=(0.93262051,0.3215093,0.24606461);
  rgb(164pt)=(0.93435067,0.32928362,0.24775328);
  rgb(165pt)=(0.93599076,0.33703942,0.24972157);
  rgb(166pt)=(0.93752831,0.34479177,0.25199928);
  rgb(167pt)=(0.93899289,0.35250734,0.25452808);
  rgb(168pt)=(0.94036561,0.36020899,0.25734661);
  rgb(169pt)=(0.94167588,0.36786594,0.2603949);
  rgb(170pt)=(0.94291042,0.37549479,0.26369821);
  rgb(171pt)=(0.94408513,0.3830811,0.26722004);
  rgb(172pt)=(0.94520419,0.39062329,0.27094924);
  rgb(173pt)=(0.94625977,0.39813168,0.27489742);
  rgb(174pt)=(0.94727016,0.4055909,0.27902322);
  rgb(175pt)=(0.94823505,0.41300424,0.28332283);
  rgb(176pt)=(0.94914549,0.42038251,0.28780969);
  rgb(177pt)=(0.95001704,0.42771398,0.29244728);
  rgb(178pt)=(0.95085121,0.43500005,0.29722817);
  rgb(179pt)=(0.95165009,0.44224144,0.30214494);
  rgb(180pt)=(0.9524044,0.44944853,0.3072105);
  rgb(181pt)=(0.95312556,0.45661389,0.31239776);
  rgb(182pt)=(0.95381595,0.46373781,0.31769923);
  rgb(183pt)=(0.95447591,0.47082238,0.32310953);
  rgb(184pt)=(0.95510255,0.47787236,0.32862553);
  rgb(185pt)=(0.95569679,0.48489115,0.33421404);
  rgb(186pt)=(0.95626788,0.49187351,0.33985601);
  rgb(187pt)=(0.95681685,0.49882008,0.34555431);
  rgb(188pt)=(0.9573439,0.50573243,0.35130912);
  rgb(189pt)=(0.95784842,0.51261283,0.35711942);
  rgb(190pt)=(0.95833051,0.51946267,0.36298589);
  rgb(191pt)=(0.95879054,0.52628305,0.36890904);
  rgb(192pt)=(0.95922872,0.53307513,0.3748895);
  rgb(193pt)=(0.95964538,0.53983991,0.38092784);
  rgb(194pt)=(0.96004345,0.54657593,0.3870292);
  rgb(195pt)=(0.96042097,0.55328624,0.39319057);
  rgb(196pt)=(0.96077819,0.55997184,0.39941173);
  rgb(197pt)=(0.9611152,0.5666337,0.40569343);
  rgb(198pt)=(0.96143273,0.57327231,0.41203603);
  rgb(199pt)=(0.96173392,0.57988594,0.41844491);
  rgb(200pt)=(0.96201757,0.58647675,0.42491751);
  rgb(201pt)=(0.96228344,0.59304598,0.43145271);
  rgb(202pt)=(0.96253168,0.5995944,0.43805131);
  rgb(203pt)=(0.96276513,0.60612062,0.44471698);
  rgb(204pt)=(0.96298491,0.6126247,0.45145074);
  rgb(205pt)=(0.96318967,0.61910879,0.45824902);
  rgb(206pt)=(0.96337949,0.6255736,0.46511271);
  rgb(207pt)=(0.96355923,0.63201624,0.47204746);
  rgb(208pt)=(0.96372785,0.63843852,0.47905028);
  rgb(209pt)=(0.96388426,0.64484214,0.4861196);
  rgb(210pt)=(0.96403203,0.65122535,0.4932578);
  rgb(211pt)=(0.96417332,0.65758729,0.50046894);
  rgb(212pt)=(0.9643063,0.66393045,0.5077467);
  rgb(213pt)=(0.96443322,0.67025402,0.51509334);
  rgb(214pt)=(0.96455845,0.67655564,0.52251447);
  rgb(215pt)=(0.96467922,0.68283846,0.53000231);
  rgb(216pt)=(0.96479861,0.68910113,0.53756026);
  rgb(217pt)=(0.96492035,0.69534192,0.5451917);
  rgb(218pt)=(0.96504223,0.7015636,0.5528892);
  rgb(219pt)=(0.96516917,0.70776351,0.5606593);
  rgb(220pt)=(0.96530224,0.71394212,0.56849894);
  rgb(221pt)=(0.96544032,0.72010124,0.57640375);
  rgb(222pt)=(0.96559206,0.72623592,0.58438387);
  rgb(223pt)=(0.96575293,0.73235058,0.59242739);
  rgb(224pt)=(0.96592829,0.73844258,0.60053991);
  rgb(225pt)=(0.96612013,0.74451182,0.60871954);
  rgb(226pt)=(0.96632832,0.75055966,0.61696136);
  rgb(227pt)=(0.96656022,0.75658231,0.62527295);
  rgb(228pt)=(0.96681185,0.76258381,0.63364277);
  rgb(229pt)=(0.96709183,0.76855969,0.64207921);
  rgb(230pt)=(0.96739773,0.77451297,0.65057302);
  rgb(231pt)=(0.96773482,0.78044149,0.65912731);
  rgb(232pt)=(0.96810471,0.78634563,0.66773889);
  rgb(233pt)=(0.96850919,0.79222565,0.6764046);
  rgb(234pt)=(0.96893132,0.79809112,0.68512266);
  rgb(235pt)=(0.96935926,0.80395415,0.69383201);
  rgb(236pt)=(0.9698028,0.80981139,0.70252255);
  rgb(237pt)=(0.97025511,0.81566605,0.71120296);
  rgb(238pt)=(0.97071849,0.82151775,0.71987163);
  rgb(239pt)=(0.97120159,0.82736371,0.72851999);
  rgb(240pt)=(0.97169389,0.83320847,0.73716071);
  rgb(241pt)=(0.97220061,0.83905052,0.74578903);
  rgb(242pt)=(0.97272597,0.84488881,0.75440141);
  rgb(243pt)=(0.97327085,0.85072354,0.76299805);
  rgb(244pt)=(0.97383206,0.85655639,0.77158353);
  rgb(245pt)=(0.97441222,0.86238689,0.78015619);
  rgb(246pt)=(0.97501782,0.86821321,0.78871034);
  rgb(247pt)=(0.97564391,0.87403763,0.79725261);
  rgb(248pt)=(0.97628674,0.87986189,0.8057883);
  rgb(249pt)=(0.97696114,0.88568129,0.81430324);
  rgb(250pt)=(0.97765722,0.89149971,0.82280948);
  rgb(251pt)=(0.97837585,0.89731727,0.83130786);
  rgb(252pt)=(0.97912374,0.90313207,0.83979337);
  rgb(253pt)=(0.979891,0.90894778,0.84827858);
  rgb(254pt)=(0.98067764,0.91476465,0.85676611);
  rgb(255pt)=(0.98137749,0.92061729,0.86536915)
},
point meta max=0.93,
point meta min=0,
tick align=outside,
tick pos=left,
title={Average Success Rate for Sparse Reward},
x grid style={darkgray176},
xlabel={Replanning Steps},
xmin=0, xmax=7,
xtick style={color=black},
xtick={0.5,1.5,2.5,3.5,4.5,5.5,6.5},
xticklabels={1,2,5,10,25,50,100},
y dir=reverse,
y grid style={darkgray176},
ylabel={Number of Basis},
ymin=0, ymax=7,
ytick style={color=black},
ytick={0.5,1.5,2.5,3.5,4.5,5.5,6.5},
yticklabel style={rotate=90.0},
yticklabels={0,1,2,3,4,5,6}
]

\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=7, ymin=7, ymax=0] {ablation_sparse_success_rate-000.png};
\draw (axis cs:0.5,0.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.00};
\draw (axis cs:1.5,0.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.00};
\draw (axis cs:2.5,0.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.00};
\draw (axis cs:3.5,0.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.04};
\draw (axis cs:4.5,0.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.13};
\draw (axis cs:5.5,0.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.03};
\draw (axis cs:6.5,0.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.00};
\draw (axis cs:0.5,1.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.24};
\draw (axis cs:1.5,1.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.38};
\draw (axis cs:2.5,1.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.70};
\draw (axis cs:3.5,1.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.40};
\draw (axis cs:4.5,1.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.62};
\draw (axis cs:5.5,1.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.40};
\draw (axis cs:6.5,1.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.05};
\draw (axis cs:0.5,2.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.57};
\draw (axis cs:1.5,2.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.88};
\draw (axis cs:2.5,2.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.82};
\draw (axis cs:3.5,2.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.89};
\draw (axis cs:4.5,2.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.78};
\draw (axis cs:5.5,2.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.35};
\draw (axis cs:6.5,2.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.15};
\draw (axis cs:0.5,3.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.78};
\draw (axis cs:1.5,3.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.88};
\draw (axis cs:2.5,3.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.90};
\draw (axis cs:3.5,3.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.93};
\draw (axis cs:4.5,3.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.72};
\draw (axis cs:5.5,3.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.67};
\draw (axis cs:6.5,3.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.38};
\draw (axis cs:0.5,4.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.74};
\draw (axis cs:1.5,4.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.89};
\draw (axis cs:2.5,4.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.89};
\draw (axis cs:3.5,4.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.92};
\draw (axis cs:4.5,4.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.93};
\draw (axis cs:5.5,4.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.73};
\draw (axis cs:6.5,4.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.65};
\draw (axis cs:0.5,5.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.69};
\draw (axis cs:1.5,5.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.84};
\draw (axis cs:2.5,5.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.68};
\draw (axis cs:3.5,5.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.81};
\draw (axis cs:4.5,5.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.93};
\draw (axis cs:5.5,5.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.72};
\draw (axis cs:6.5,5.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.61};
\draw (axis cs:0.5,6.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.59};
\draw (axis cs:1.5,6.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.66};
\draw (axis cs:2.5,6.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.51};
\draw (axis cs:3.5,6.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.71};
\draw (axis cs:4.5,6.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.88};
\draw (axis cs:5.5,6.5) node[
  scale=0.5,
  text=darkslategray38,
  rotate=0.0
]{0.89};
\draw (axis cs:6.5,6.5) node[
  scale=0.5,
  text=white,
  rotate=0.0
]{0.57};
\end{axis}

\end{tikzpicture}

==> util/Math_Symbols.tex <==
\section{Symbols}
\renewcommand{\arraystretch}{1.33}
% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
\begin{table}[htbp]
    \small
    \centering
    % \vspace{-0.7cm}
    \caption{List of symbols used in this paper.\vspace{0.2cm}}
    \begin{tabular}{cm{12.8cm}}
        \toprule
        \textbf{Symbol} & \textbf{Description}\\
        \hline
        $ \bm{a} $ & The action being taken at each single time \\
        $ A $ & The advantage \\
        $ b $ & The time step of the initial conditions \\
        $ c $ & Coefficients of the complementary solutions of \acrshortpl{dmp}' \acrshort{ode} \\
        $ d,~D $ & Index and the number of \acrshortpl{dof} \\
        $ f $ & Forcing function of the original \acrshortpl{dmp} \\
        $ F $ & The source term in the \acrshortpl{dmp}'non-homogeneous \acrshortpl{ode} \\
        $ g $ & The Goal term of \acrshortpl{dmp} and \acrshortpl{pdmp}\\
        % % $ h $ & index used to describe the time indices \\
        % $ \bm{H} $ & A combination of \acrshortpl{pdmp}' basis and boundary conditions terms, used in distribution computation \\
        % $ i $ & Index of the basis functions and weights of one \acrshort{dof}\\
        % $ j,~J $ & Index and the total number of the randomly selected time pairs used in loss computation \\
        $ J $ & RL objective\\
        % $ k $ & Index of the boundary condition terms \\
        % $ I $ & The two indefinite integrals in the closed form solution of \acrshortpl{dmp}' \acrshort{ode} \\
        % $ l $ & The length of a trajectory segment \\
        % $ L $ & The number of trajectory segments in a whole trajectory \\
        % $ \mathscr{L} $ & The total length of a trajectory $\sum_{h=0}^{L-1}l_h$ \\
        % $ \mathcal{L} $ & The lower-diagonal Cholesky decomposition of a covariance matrix \\
        % $ N $ & The number of basis functions and weights per \acrshortpl{dof}  \\
        % $ N $ & The number of sampled trajectories\\
        % $ m,~M $ & Index and the number of observations \\
        % $ \bm{o},~\mathcal{O} $ & Sensory observation and a set of observations \\
        % $ \bm{p} $ & The first definite integral in $I$ which must be computed using a numerical integral \\
        % $ q $ & The second definite integral in $I$ which can be solved analytically\\
        % $ \bm{r} $ & Latent observation \\
        $ r, R $ & The reward and the return \\
        % $ \bm{s} $ & The state of each single time step, low level  \\
        % $ \bm{S} $ & The state of each trajectory segment, high level,   \\
        $ t $ & index of time steps\\
        % $ T $ & High-level index of trajectory segments in a whole trajectory\\
        $ \bm{w}, \bm{w_g} $ & The weights of \acrshortpl{dmp}, \acrshortpl{promp}, and \acrshortpl{pdmp}. A concatenation of weights and goal.\\
        % $ x $ & The phase of the canonical system, which decays exponentially w.r.t time. \\
        $ y, ~\dot{y},~ \ddot{y} $ & One \acrshort{dof} trajectory position, velocity, and acceleration of a single time step respectively \\
        $ \bm{y} $ & $D$-\acrshortpl{dof} trajectory position of a single time step \\
        $ V $ & The value function\\
        $ Q $ & The state-action value function\\
        % $ Y $ & The denominator in the indefinite integrals $I_1$ and $I_2$\\
        % $ \bm{z} $ & The latent variable in Neural Processes, Bayesian Aggregation and \acrshortpl{pdmp}' deep embeddings \\
        \midrule
        % $ \alpha_x $ & Exponential decaying coefficient of the canonical system \\
        $ \alpha $ & Learning rate \\
        % $ \alpha, \beta $ & Spring-damper coefficient of \acrshortpl{dmp}  \\
        % $ \Delta  $ & The characteristic equation of \acrshortpl{dmp}' homogeneous \acrshortpl{ode}\\
        % $ \epsilon $ & Gaussian white noise \\
        $ \theta $ & Neural Networks' learnable parameters \\
        $ \bm{\lambda}, \bm{\Lambda} $ & A single \acrshort{dof} trajectory and a multi \acrshortpl{dof} trajectory \\
        % $ \mu, \bm{\mu} $ & The mean of a certain probabilistic distribution \\
        % $ \xi,~\bm{\xi} $ & One or multi time-step term determined by boundary conditions in \acrshortpl{pdmp}' trajectory computation \\
        % % $ \pi $ &  \\
        $ \pi $ & The policy  \\
        % $ \rho $ & Low-level index of time steps in a trajectory segment\\
        $ \gamma $ & The reward discount factor  \\
        % $ \sigma^2 $ & The variance of a certain probabilistic distribution \\
        % $ \bm{\Sigma} $ & The covariance of a certain probabilistic distribution \\
        % $ \tau $ & Time scaling factor of \acrshortpl{dmp}, determining the execution speed \\
        $ \tau $ & the time factor used in \acrshort{pdmp} to adjust the trajectory speed.\\
        % $ \bm{\varphi} $ & Basis function forming up \acrshortpl{dmp}' forcing term \\
        % $ \bm{\Phi} $ & Basis functions of one \acrshort{dof} used by \acrshortpl{promp} and \acrshortpl{pdmp}, written in matrix \\
        % $ \bm{\Psi} $ & Blocked diagonal basis function matrix used by \acrshortpl{promp} and \acrshortpl{pdmp} for multi \acrshortpl{dof} trajectory \\
        % $ \dot{\bm{\Phi}}, \dot{\bm{\Psi}} $ & Single and blocked diagonal velocity basis function matrices \\
        % $  $ &  \\
        \bottomrule
    \end{tabular}
     \vspace{-.5cm}
    \label{tab:model_comparison}
\end{table}
\renewcommand{\arraystretch}{1}

% \renewcommand{\arraystretch}{1.33}
% % \setlength{\aboverulesep}{0pt}
% % \setlength{\belowrulesep}{0pt}
% \begin{table}[htbp]
%     \small
%     \centering
%     % \vspace{-0.7cm}
%     \caption{Ref: List of symbols used in ProDMP paper.\vspace{0.2cm}}
%     \begin{tabular}{cm{12.8cm}}
%         \toprule
%         \textbf{Symbol} & \textbf{Description}\\
%         \hline
%         $ b $ & The time step of the boundary conditions \\
%         $ c $ & Coefficients of the general solutions of \acrshortpl{dmp}' \acrshort{ode} \\
%         $ d,~D $ & Index and the number of \acrshortpl{dof} \\
%         $ f $ & Forcing function of the original \acrshortpl{dmp} \\
%         $ F $ & The source term in the \acrshortpl{dmp}'non-homogeneous \acrshortpl{ode} \\
%         $ g $ & The Goal term of \acrshortpl{dmp} and \acrshortpl{pdmp}\\
%         % $ h $ &  \\
%         $ \bm{H} $ & A combination of \acrshortpl{pdmp}' basis and boundary conditions terms, used in distribution computation \\
%         $ i $ & Index of the basis functions and weights of one \acrshort{dof}\\
%         $ j,~J $ & Index and the total number of the randomly selected time pairs used in loss computation \\
%         $ k $ & Index of the boundary condition terms \\
%         $ I $ & The two indefinite integrals in the closed form solution of \acrshortpl{dmp}' \acrshort{ode} \\
%         $ \bm{L} $ & The Cholesky decomposition of a covariance matrix \\
%         $ \mathcal{L} $ & The loss function to be minimized \\
%         $ N $ & The number of basis functions and weights per \acrshortpl{dof}  \\
%         $ m,~M $ & Index and the number of observations \\
%         $ \bm{o},~\mathcal{O} $ & Sensory observation and a set of observations \\
%         $ \bm{p} $ & The first definite integral in $I$ which must be computed using a numerical integral \\
%         $ q $ & The second definite integral in $I$ which can be solved analytically\\
%         $ \bm{r} $ & Latent observation \\
%         $ t, T $ & Index of time steps and the length of trajectory, i.e. the number of total time steps \\
%         $ \bm{w}, \bm{w_g} $ & The weights of \acrshortpl{dmp}, \acrshortpl{promp}, and \acrshortpl{pdmp}. A concatenation of weights and goal.\\
%         $ x $ & The phase of the canonical system, which decays exponentially w.r.t time. \\
%         $ y, ~\dot{y},~ \ddot{y} $ & One \acrshort{dof} trajectory position, velocity, and acceleration of a single time step respectively \\
%         $ \bm{y} $ & $D$-\acrshortpl{dof} trajectory position of a single time step \\
%         $ Y $ & The denominator in the indefinite integrals $I_1$ and $I_2$\\
%         $ \bm{z} $ & The latent variable in Neural Processes, Bayesian Aggregation and \acrshortpl{pdmp}' deep embeddings \\
%         \midrule
%         $ \alpha_x $ & Exponential decaying coefficient of the canonical system \\
%         $ \alpha, \beta $ & Spring-damper coefficient of \acrshortpl{dmp}  \\
%         $ \Delta  $ & The characteristic equation of \acrshortpl{dmp}' homogeneous \acrshortpl{ode}\\
%         $ \epsilon $ & Gaussian white noise \\
%         $ \theta $ & Neural Networks' learnable parameters \\
%         $ \bm{\lambda}, \bm{\Lambda} $ & A single \acrshort{dof} trajectory and a multi \acrshortpl{dof} trajectory \\
%         $ \mu, \bm{\mu} $ & The mean of a certain probabilistic distribution \\
%         $ \xi,~\bm{\xi} $ & One or multi time-step term determined by boundary conditions in \acrshortpl{pdmp}' trajectory computation \\
%         % $ \pi $ &  \\
%         $ \sigma^2 $ & The variance of a certain probabilistic distribution \\
%         $ \bm{\Sigma} $ & The covariance of a certain probabilistic distribution \\
%         $ \tau $ & Time scaling factor of \acrshortpl{dmp}, determining the execution speed \\
%         $ \bm{\varphi} $ & Basis function forming up \acrshortpl{dmp}' forcing term \\
%         $ \bm{\Phi} $ & Basis functions of one \acrshort{dof} used by \acrshortpl{promp} and \acrshortpl{pdmp}, written in matrix \\
%         $ \bm{\Psi} $ & Blocked diagonal basis function matrix used by \acrshortpl{promp} and \acrshortpl{pdmp} for multi \acrshortpl{dof} trajectory \\
%         $ \dot{\bm{\Phi}}, \dot{\bm{\Psi}} $ & Single and blocked diagonal velocity basis function matrices \\
%         % $  $ &  \\
%         \bottomrule
%     \end{tabular}
%      \vspace{-.5cm}
%     \label{tab:model_comparison}
% \end{table}
% \renewcommand{\arraystretch}{1}
